Effects of symmetry and hydrodynamics on the cohesion of groups of swimmers

When groups of inertial swimmers move together, hydrodynamic interactions play a key role in shaping their collective dynamics, including the cohesion of the group. To explore how these interactions influence group cohesion, we develop a three-dimensional, inviscid, far-field model of a swimmer. Focusing on symmetric triangular, diamond, and circular group arrangements, we investigate whether passive hydrodynamics alone can promote cohesive behavior, and what role symmetry of the group plays. While small symmetric (and even asymmetric) groups can be cohesive, larger groups typically are not, instead breaking apart into smaller, self-organized subgroups that are cohesive. Notably, we discover circular arrangements of swimmers that chase each other around a circle, resembling the milling behavior of natural fish schools; we call this hydrodynamic milling. Hydrodynamic milling is cohesive in the sense that it is a fixed point of a particular Poincar\'e map, but it is unstable, especially to asymmetric perturbations. Our findings suggest that while passive hydrodynamics alone cannot sustain large-scale cohesion indefinitely, controlling interactions between subgroups, or controlling the behavior of only the periphery of a large group, could potentially enable stable collective behavior with minimal active input.

==> rings.tex <==
We also study circular configurations in different settings. One such setup is the \emph{nested arrangement}, where $2N$ swimmers are uniformly distributed across two concentric circles of radii $R_1 = 2.5$ and $R_2 = 4$, as illustrated in Figure~\ref{fig:nested}. In this configuration, the group destabilizes more rapidly compared to the single-ring arrangement. The swimmers pair up and exhibit a coordinated, braid-like motion. When compared to the standard milling dynamics, we observe that the difference in radii between the two rings accelerates the transition from collective rotation to pairwise interactions. Despite the instability of the global configuration, the pairwise motion remains robust and characterizes the long-term dynamics of the system.

\begin{figure}[!h]
    \centering
      \subfigure[]{
      \includegraphics[width=0.45\textwidth]{Nested_milling.pdf}
      \label{fig:configurationnested}
      }
      \subfigure[]{
        \includegraphics[width=0.45\textwidth]{Picture12.pdf}
        \label{fig:traject}
      }
    \caption{\label{fig:nested} (a)~ Arrangement of two concentric circles of radii $R_1 = 2.5$ and $R_2 = 4.0$. (b)~ Planar trajectories.}
\end{figure}

Another three-dimensional arrangement we investigate involves two \emph{coaxial rings}, each of radius $R = 2.5$, positioned in planes $z = +d$ and $z = -d$ where $d = 2.0$, respectively. A total of $2N$ swimmers are placed on these rings, all oriented in the positive $z$-direction; see Figure~\ref{fig:rings}. Similar to the nested circle case, this configuration also leads to the formation of robust, braided trajectories. The swimmers pair up and maintain these intertwined paths over long time scales, indicating that the braided interaction is a recurring stable structure in both planar and three-dimensional multi-ring configurations.

\begin{figure}[!h]
    \centering
      \subfigure[]{
      \includegraphics[width=0.45\textwidth]{Picture3.pdf}
      \label{fig:configurationrings}
      }
      \subfigure[]{
        \includegraphics[width=0.45\textwidth]{Picture13.pdf}
        \label{fig:trajectrings}
      }
    \caption{\label{fig:rings} a)~ Arrangement of two coaxial rings separated by $2d$ in the z-direction. (b)~Three dimensional trajectories of the swimmers.}
\end{figure}

